Neural basis expansion analysis with exogenous variables: Forecasting electricity prices with NBEATSx

We extend the neural basis expansion analysis (NBEATS) to incorporate exogenous factors. The resulting method, called NBEATSx, improves on a well performing deep learning model, extending its capabilities by including exogenous variables and allowing it to integrate multiple sources of useful information. To showcase the utility of the NBEATSx model, we conduct a comprehensive study of its application to electricity price forecasting (EPF) tasks across a broad range of years and markets. We observe state-of-the-art performance, significantly improving the forecast accuracy by nearly 20% over the original NBEATS model, and by up to 5% over other well established statistical and machine learning methods specialized for these tasks. Additionally, the proposed neural network has an interpretable configuration that can structurally decompose time series, visualizing the relative impact of trend and seasonal components and revealing the modeled processes' interactions with exogenous factors. To assist related work we made the code available in https://github.com/cchallu/nbeatsx.

==> sections/section3_nbeatsx_new.tex <==
As a general overview, the \NBEATSx \ framework decomposes the objective signal by performing separate local nonlinear projections of the data onto basis functions across its different blocks. Figure~\ref{fig:nbeatsx_architecture} depicts the general architecture of the model. Each block consists of a \emph{Fully Connected Multi Layer Perceptron} (\MLP; \citealt{rosenblatt1961principles}) which learns expansion coefficients for the backcast and forecast elements. The backcast model is used to clean the inputs of subsequent blocks, while the forecasts are summed to compose the final prediction. The blocks are grouped in stacks. Each of the potentially multiple stacks specializes in a different variant of basis functions.

\begin{figure}[!ht] %tb
\centering
\includegraphics[width=1.0\linewidth]{images/NBEATSX.pdf}
\caption{Building blocks of the \NBEATSx\ are structured as a system of multilayer fully connected networks with ReLU based nonlinearities. 
Blocks overlap using the doubly residual stacking principle for the backcast $\mathbf{\tilde{y}}_{[t-L:t],s,b}$ and forecast $\mathbf{\hat{y}}_{[t+1:t+H],s,b}$ outputs of the $b$-th block within the $s$-th stack. The final predictions $\mathbf{\hat{y}}_{[t+1:t+H]}$ are composed by aggregating the outputs of the stacks.
} \label{fig:nbeatsx_architecture} % \KO{Improved description and Figure with s,b indexes}
\end{figure}

To continue the description of the \NBEATSx, we introduce the following notation: the objective signal is represented by the vector $\mathbf{y}$, the inputs for the model are the backcast window vector $\mathbf{y}_{[t-L:t]}$ of length $L$, and the forecast window vector $\mathbf{y}_{[t+1:t+H]}$ of length $H$; where $L$ denotes the length of the lags available as classic autoregressive features, and $H$ is the forecast horizon treated as the objective. While the original \NBEATS\ only admits as regressor the backcast period of the target variable $\mathbf{y}_{[t-L:t]}$, the \NBEATSx\ incorporates covariates in its analysis denoted with the matrix $\mathbf{X}$. Figure~\ref{fig:nbeatsx_architecture} shows an example where the target variable is the hourly electricity price,  the backcast vector has a length $L$ of 96 hours, and the forecast horizon $H$ is 72 hours, in the example, the covariate matrix $\mathbf{X}$ is composed of wind power production and electricity load. For the EPF comparative analysis of Section~\ref{subsection:forecasting_results} the horizon considered is $H=24$ that corresponds to day-ahead predictions, while backcast inputs $L=168$ correspond to a week of lagged values.

%\KO{Addressed local inputs inquiry from Reviewer 1}
For its predictions, the \NBEATSx\ model only receives a local vector of inputs corresponding to the backcast period, making the computations exceptionally fast. The model can still represent longer time dependencies through its local inputs from the exogenous variables; for example, it can learn long seasonal effects from calendar variables. Overall, as shown in Figure~\ref{fig:nbeatsx_architecture}, the \NBEATSx\ is composed of $S$ stacks of $B$ blocks each, the input $\mathbf{y}_{[t-L:t]},\mathbf{X}_{[t-L:t]}$ of the first block consists of $L$ lags of the target time series $\mathbf{y}$ and the exogenous matrix $\mathbf{X}$, while the inputs of each of the subsequent blocks include residual connections with the backcast output of the previous block. We will describe in detail in the next subsections the blocks, stacks, and model predictions.

% \clearpage
\subsection{Blocks}

%\KO{Improvements to notation to depend on stack and blocks s,b indexes}
For a given $s$-th stack and $b$-th block within it, the \NBEATSx\ model performs two transformations, depicted in the blue rectangle of Figure~\ref{fig:nbeatsx_architecture}. The first transformation, defined in Equation~(\ref{equation:block_transformations1}) and (\ref{equation:block_transformations2}), takes the input data $(\mathbf{y}_{[t-L:t],s,b-1}, \mathbf{X}_{[t-L:t+H],s})$, and applies a \emph{Fully Connected Multi Layer Perceptron} (\MLP; \citealt{rosenblatt1961principles}) to learn hidden units $\mathbf{h}_{s,b} \in \mathbb{R}^{N_{h}}$ that are linearly adapted into the forecast $\btheta^{f}_{s,b} \in \mathbb{R}^{N_{st}}$ and backcast $\btheta^{b}_{s,b}\in \mathbb{R}^{N_{st}}$ expansion coefficients, with $N_{st}$ the dimension of the stack basis.

\begin{equation}
    \mathbf{h}_{s,b} = \mathbf{MLP}_{s,b}\left(\mathbf{y}_{[t-L:t],s,b}\right)
    \quad \text{or} \quad 
    \mathbf{h}_{s,b} = \mathbf{MLP}_{s,b}\left(\mathbf{y}_{[t-L:t],s,b}, \mathbf{X}_{[t-L:t+H],s}\right)
    \label{equation:block_transformations1}
\end{equation}

\begin{equation}
    \btheta^{b}_{s,b} = \textbf{LINEAR}^{b}\left(\mathbf{h}_{s,b}\right) 
    \quad \text{and} \quad
    \btheta^{f}_{s,b} = \textbf{LINEAR}^{f}\left(\mathbf{h}_{s,b}\right)
    \label{equation:block_transformations2}
\end{equation}

% \KO{Simplified Eq (2) with matrix notation and defined dimensions}
The second transformation, in Equation~(\ref{equation:nonlinear_projections}), consists of a basis expansion between the learnt coefficients and the block's basis $\mathbf{V}_{[t-L:t],s,b} \in \mathbb{R}^{L \times N_{st}}$ and $\mathbf{V}_{[t+1:t+H],s,b} \in \mathbb{R}^{H \times N_{st}}$, this transformation results in the backcast $ \mathbf{\tilde{y}}_{[t-L:t],s,b}$ and forecast $\mathbf{\hat{y}}_{[t+1:t+H],s,b}$ components.

\begin{equation}
    \mathbf{\tilde{y}}_{[t-L:t],s,b} 
    = \mathbf{V}_{[t-L:t],s,b} \, \btheta^{b}_{s,b}
    \quad \text{and} \quad
    \mathbf{\hat{y}}_{[t+1:t+H],s,b} 
    = \mathbf{V}_{[t+1:t+H],s,b} \,\btheta^{f}_{s,b}
    \label{equation:nonlinear_projections}
\end{equation}

\subsection{Stacks and Residual Connections}

%\KO{Added subsection of stacks and residual connections}
The blocks are organized into stacks using the doubly residual stacking principle, which is described in Equation~(\ref{equation:stacks_connections}) and depicted in the brown rectangle of Figure~\ref{fig:nbeatsx_architecture}. The residual backcast $\mathbf{y}_{[t-L:t],s,b+1} \in \mathbb{R}^{L}$ allows the model to subtract the component associated to the basis of the $s,b$-th stack and block $\mathbf{V}_{[t-L:t]s,b}$ from $\mathbf{y}_{[t-L:t]}$, which can be also thought of as a sequential decomposition of the modeled signal. In turn, this methodology helps with the optimization procedure as it prepares the inputs of the subsequent layer making the downstream forecast easier. The stack forecast $\hat{\mathbf{y}}_{[t+1:t+H],s}  \in \mathbb{R}^{H}$ aggregates the partial forecasts from each block.
\begin{equation}
% \color{blue}
    \mathbf{y}_{[t-L:t],s,b+1} = \mathbf{y}_{[t-L:t],s,b}-\mathbf{\tilde{y}}_{[t-L:t],s,b} 
    \qquad \text{and} \qquad
    \mathbf{\hat{y}}_{[t+1:t+H],s}
    = \sum^{B}_{b=1} \hat{\mathbf{y}}_{[t+1:t+H],s,b}
    \label{equation:stacks_connections}
\end{equation}

%\newpage
\subsection{Model predictions}

%\KO{Added subsection of final model predictions}
The final predictions $\hat{\mathbf{y}}_{[t+1:t+H]} \in \mathbb{R}^{H}$, we later denote the predictions for a particular day as $\hat{\mathbf{y}}_{d}$, shown in the yellow rectangle of Figure~\ref{fig:nbeatsx_architecture}, are obtained by summation of all the stack predictions.
\begin{equation}
    \mathbf{\hat{y}}_{[t+1:t+H]} 
    %= \sum^{S}_{s=1} \left(\sum^{B}_{b=1} \hat{\mathbf{y}}^{for}_{s,b} \right) 
    = \sum^{S}_{s=1} \hat{\mathbf{y}}_{[t+1:t+H],s} 
    %= \sum^{S}_{s=1} (\sum^{B}_{b=1} \hat{\mathbf{y}}^{for}_{s,b})
    \label{equation:predictions}
\end{equation}

The additive generation of the forecast implies a very intuitive decomposition of the prediction components when the bases within the blocks are interpretable.

\clearpage
\subsection{NBEATSx Configurations}
\label{subsection:nbeatsx_configurations}

The original \emph{neural basis expansion analysis} method proposed two configurations based on the assumptions encoded in the learning algorithm by selecting the basis vectors $\mathbf{V}_{[t-L:t],s,b}$ and $ \mathbf{V}_{[t+1:t+H],s,b}$ used in the blocks from Equation~(\ref{equation:nonlinear_projections}). A mindful selection of restrictions to the basis allows the model to output an interpretable decomposition of the forecasts, while allowing the basis to be freely determined can produce more flexible forecasts by effectively removing any constraints on the form of the basis functions. 

In this subsection, we present both interpretable and generic configurations, explaining in particular how we propose to include the covariates in each case. We limit ourselves to the analysis of the forecast basis, as the backcast basis analysis is almost identical, only differing by its extension over time. We show an example in \ref{appendix:basis}. 
%\KO{Address concern of Reviewer 1, backcast basis mentioned here and in Appendix.}

\subsubsection{Interpretable Configuration}
\label{subsubsection:nbeatsx_configurations}

% RW --> I have reduced the number of cited Refs
The choice of basis vectors relies on time series decomposition techniques that are often used to understand the structure of a given time series and patterns of its variation. 
Work in this area ranges from classical smoothing methods 
%\citep{mcaulay1930smoothing} 
and their extensions such as X-11-\ARIMA, 
%\citep{shishkin1967x11, dagum1980x11arima}, 
X-12-\ARIMA, 
%\citep{x12arima}, 
and X-13-\ARIMA-\SEATS, 
%\citep{x13seats}, 
to modern approaches such as \TBATS~\citep{hyndman2011tbats}.
%and STR \citep{dokumentov2020str}.
%STL \citep{cleveland1990STL}
To encourage interpretability, the blocks within each stack may use harmonic functions, polynomial trends, and exogenous variables directly to perform their projections. 
The partial forecasts of the interpretable configuration are described by Equations~(\ref{equation:interpretable_trend})-(\ref{equation:interpretable_exogenous}).
%\KO{Changed notation to include s,b indexes}

\begin{equation}
% \color{blue}
    \hat{\mathbf{y}}^{trend}_{[t+1:t+H],s,b} 
    = \sum^{N_{pol}}_{i=0} \mathbf{t}^{i}  \; \theta^{trend}_{s,b,i}
    \equiv \mathbf{T} \; \btheta^{trend}_{s,b}
\label{equation:interpretable_trend}
\end{equation}

\begin{equation}
% \color{blue}
    \hat{\mathbf{y}}^{seas}_{[t+1:t+H],s,b} 
    = \sum^{N_{har}}_{i=0} \cos\left(2\pi i \mathbf{t}\right) \theta^{seas}_{s,b,i} + \sin \left( 2\pi i \mathbf{t}\right) \theta^{seas}_{s,b,i+\lfloor H/2 \rfloor} 
    \equiv  \mathbf{S} \; \btheta^{seas}_{s,b} %\lfloor H/2 -1 \rfloor
\label{equation:interpretable_seasonality}
\end{equation}

\begin{equation}
% \color{blue}
    \hat{\mathbf{y}}^{exog}_{[t+1:t+H],s,b} 
    = \sum^{N_x}_{i=0} \mathbf{X}_{[t+1:t+H],i} \, \theta^{exog}_{s,b,i}
    \equiv \mathbf{X}_{[t+1:t+H]} \; \btheta^{exog}_{s,b}  
\label{equation:interpretable_exogenous}
\end{equation}
where the time vector $\mathbf{t}^{\intercal}=[0,1,2,\dots,H-2, H-1]/H$ is defined discretely.  When the basis $ \mathbf{V}_{[t+1:t+H],s,b}$ is $ \mathbf{T}=[\mathbf{1},\mathbf{t},\dots,\mathbf{t}^{N_{pol}}] \in \mathbb{R}^{H \times (N_{pol}+1)}$, where $N_{pol}$ is the maximum polynomial degree, the coefficients are those of a polynomial model for the trend. When $\mathbf{V}_{[t+1:t+H],s,b}$ are harmonic $ \mathbf{S}=[\mathbf{1},\cos(2\pi \mathbf{t}),\dots, \cos(2 \pi i \mathbf{t}), \sin(2\pi \mathbf{t}),\dots,\sin(2 \pi i \mathbf{t})] \in \mathbb{R}^{H \times N_{har}} $, and $N_{har}=(H-1)$, the coefficients vector $ \btheta^{f}_{s,b}$ can be interpreted as Fourier transform coefficients. The exogenous basis expansion can be thought as a time-varying local regression when the basis is the matrix $ \mathbf{X}_{[t+1:t+H]}=[\mathbf{X}_{1},\dots,\mathbf{X}_{N_x}] \in \mathbb{R}^{H \times N_x} $, where $N_{x}$ is the number of exogenous variables. The resulting models can flexibly reflect common structural assumptions, in particular using the interpretable bases, as well as their combinations. 
%\KO{Changed the equations order, improved introduction, added dimensions}

\newpage
In this paper, we propose including one more type of stack to specifically represent exogenous variable basis as described in Equation~(\ref{equation:interpretable_exogenous}) and depicted in Figure~\ref{fig:nbeatsx_architecture}. 
In the original \NBEATS\ framework~(\cite{oreshkin2020nbeats}), the interpretable configuration usually consists of a trend stack followed by a seasonality stack, each containing three blocks. 
Our \NBEATSx\ extension of this configuration consists of three stacks, one of each type of factors (trend, seasonal, exogenous). 
We refer to this interpretable and its enhanced interpretable configuration as the \NBEATSi\ and \NBEATSxi\ models, respectively.
%\KO{Here is the introduction to NBEATSx-I and NBEATS-I}

%\newpage
\subsubsection{Generic Configuration}

%\KO{Improved introduction of equation and changed order of equation} 
%\KO{Improved description of Equation 7 by moving identity and horizon dimension definitions closer.}
For the generic configuration, the basis of the non linear projection in Equation~(\ref{equation:nonlinear_projections}) corresponds to canonical vectors, that is $\mathbf{V}_{[t+1:t+H],s,b} = I_{H \times H}$,  an identity matrix of dimensionality equal to the forecast horizon $H$ that matches the coefficient's cardinality $ |\btheta^{f}_{s,b}| = H$. 
\begin{equation}
\begin{aligned}
    \mathbf{\hat{y}}_{[t+1:t+H],s,b} 
    = \mathbf{V}_{[t+1:t+H],s,b} \; \btheta^{f}_{s,b} 
    = \btheta^{f}_{s,b}
    \label{equation:generic_basis}
\end{aligned}
\end{equation}

This basis enables \NBEATSx \ to effectively behave like a classic \emph{Fully Connected Multilayer Perceptron} (\MLP).
The output layer of the \MLP \ inside each block has $H$ neurons, that correspond to the forecast horizon, each producing the forecast for one particular time point of the forecast period. This can be understood as the basis vectors being learned during optimization, allowing the waveform of the basis of each stack to be freely determined in a data-driven fashion. Compared to the interpretable counterpart described in Section~\ref{subsubsection:nbeatsx_configurations}, the constraints on the form of the basis functions are removed. This affords the generic variant more flexibility and power at representing complex data, but it can also lead to less interpretable outcomes and potentially escalated risk of overfitting.

For the \NBEATSx \ model with the generic configuration, we propose a new type of exogenous block that encodes the past $\mathbf{C}_{[t+1:t+H],s,b} \in \mathbb{R}^{H\times N_{f}}$ from the time-dependent covariates with an \textit{encoder} convolutional sub-structure:
\begin{equation}
\begin{aligned}
    \hat{\mathbf{y}}^{exog}_{[t+1:t+H],s,b} 
    = \sum^{N_{f}}_{i=1} C_{[t+1:t+H],s,b,i} \;\theta^{f}_{s,b,i} 
    \equiv \mathbf{C}_{[t+1:t+H],s,b} \;\btheta^{f}_{s,b} \\
    \qquad \text{with} \qquad
    \mathbf{C}_{[t+1:t+H],s,b} = \text{TempConv}(\mathbf{X}_{[t-L:t+H],s})_{[t+1:t+H]} 
    \label{equation:exogenous_encoder}
\end{aligned}
\end{equation}
In the previous equation, a \emph{Temporal Convolutional Network} (\TempConv;~\citealt{zico2018tcnn, vandenoord2016wavenet}) is employed as an \emph{encoder}, but any neural network with a sequential structure will be compatible with the backcast and forecast branches of the model, and could be used as an \emph{encoder}. Temporal convolutions can be an effective alternative to RNNs as it is also able to capture long term dependencies and interactions of covariates by stacking multiple layers, while dilations help it keep the models computationally tractable. In addition, convolutions have a very convenient interpretation as a weighted moving average signal filters. The final linear projection and the additive composition of the predictions can be interpreted as a \emph{decoder}. The original NBEATS configuration includes only one generic stack with dozens of blocks, while our proposed model includes both the generic and exogenous stacks, with the order determined via data-driven hyperparameter tuning. We refer to this configuration as the \NBEATSxg \ model.




\subsubsection{Exogenous Variables}

%\KO{Simplified Exogenous Variables section, eliminated two references}

%\KO{Assert that trend and harmonic functions could be understood as exogenous}

%This subsection briefly discusses different types of exogenous variables and how we can incorporate them in our proposed NBEATSx model. 
We distinguish the exogenous variables by whether they reflect static or time-dependent aspects of the modeled data.
%
The \emph{static} exogenous variables carry time-invariant information. When the model is built with common parameters to forecast multiple time series, these variables allow sharing information within groups of time series with similar static variable levels. Examples of static variables include designators such as identifiers of regions, groups of products, among others. 

As for the \emph{time-dependent} exogenous covariates, we discern two subtypes. First, we consider seasonal covariates from the natural frequencies in the data. These variables are useful for \NBEATSx \ to identify seasonal patterns and special events inside and outside the window lookback periods. Examples of these are the trends and harmonic functions from Equation~(\ref{equation:interpretable_trend}) and Equation~(\ref{equation:interpretable_seasonality}). Second, we identify domain-specific temporal covariates unique to each problem. The EPF setting typically includes day-ahead forecasts of electricity load and production levels from renewable energy sources.

%This subsection briefly discusses different types of exogenous variables and how they are incorporated by our proposed NBEATSx method. We distinguish the exogenous variables by whether they reflect static or time-dependent aspects of the modeled data.

%The static exogenous variables carry time-invariant information. When the model is built with common parameters to forecast multiple time series, these variables allow sharing information within groups of time series with similar static variable levels. Examples of static variables include designators such as identifiers of regions, groups of products, etc., that can be used to mark agglomerates of series that demonstrate similar behaviors.
%Since the static variables are used as inputs of the FCNN in each block, the NBEATSx allows for interactions between the static and temporal variables.

%As for the time-dependent exogenous covariates, we discern two subtypes. First, we consider seasonal covariates that are linked to the natural frequencies in the data. 
%In the EPF example, these variables include calendar variables to identify hours, days, months, or holidays, among others. They can be implemented using one-hot-encoded vectors of indicators or linear kernels centered around holidays, or days of the week. Linear kernels are inspired by the \emph{Generalized Additive Model} (GAM) heuristics from the time series literature \citep{evgeniou2000rkhs_regression, gaillard2016gefcom2014}.
%These variables are useful for NBEATSx to identify seasonal patterns and special events outside the window lookback periods. 
%They can also help the models reflect sharp contrasts induced by discrete events or apparent change-points, which are hard to represent well using smooth bases such as polynomial or harmonic functions.

%Finally, we identify domain-specific temporal covariates which can be unique to each problem. These variables are usually known to affect the target variable fundamentally and need to be incorporated by models to produce accurate forecasts. In the EPF setting, they typically include day-ahead forecasts of electricity load and production levels from renewable energy sources.
%Time-dependent covariates are included as inputs of the FCNN in all blocks and basis vectors for the blocks in the exogenous stack, as explained in Section \ref{section:model}.


==> sections/section5_discussion.tex <==
Neural basis expansion analysis is a flexible and powerful framework for advanced forecast modeling, yet we identified some limitations and other interesting questions that arose from our empirical evaluations. 
First, the observed improvements pertain to point forecasts only, while other models, such as the ESRNN, already offer probabilistic forecasts. Second, the generic NBEATSx-G and interpretable NBEATSx-I configurations did not show significant differences in their performance on the selected benchmark tests. This raises an interesting question on the possibility of the simpler interpretable model outperforming the generic counterpart on scarce data settings by being more robust to overfitting and by using specialized alternative basis expansions tailored to the problem at hand. Further research on the use of neural networks for time series forecasting in scarce data settings can overcome their limitations and further their adoption in practice. 

Below, we elaborate on a few ideas that we believe could help to further expand the applications of NBEATSx. These extension ideas address first the outputs and functionalities of the model, and second the challenge of data scarcity that is exacerbated by the large number of adaptable parameters in the model.

\subsection{Probabilistic Forecasts}

NBEATSx can be extended towards probabilistic forecasting using a similar approach to that of quantile regression. 
Without selecting a particular distribution, one can precisely estimate quantiles of the sample distribution by simply changing the training objective function from the mean absolute error (MAE) to the quantile loss \citep{koenker_basset1978quantile_regression, uniejewski2021quantile_reg}. This approach has the additional benefit of providing robustness to outliers and noise in the data. In some cases, it may even be used to reduce systemic biases in the forecasts \citep{smyl2019esrnn}.
% \begin{equation}
%     QL_{q} = \frac{1}{24 N_{d}} \sum^{N_{d}}_{d=1}\sum^{24}_{h=1}\left(q\left(y_{d,h}-\hat{y}_{d,h}\right)_{+}+(1-q)\left(\hat{y}_{d,h}-y_{d,h}\right)_{+}\right)
% \end{equation}

% \subsection{Interventions}
% Causal effects added into the covariates $\mathbf{X}$ matrix inputs of the model.
% \cite{box_tiao1975interventions}

\subsection{Alternative Basis Expansions}

As an alternative to the use of one dimensional convolutions in the exogenous covariate encoders, the interpretable configuration of NBEATSx could use other transformations to filter and extract useful features from data. Instead of using the convolutional weighted average procedure from Equation~(\ref{equation:exogenous_encoder}), one can use smoothing alternatives such as splines \citep{hastie1986gams, friedman1991mars}. As an alternative to Fourier projections from Equation~(\ref{equation:interpretable_exogenous}) one could also explore the wavelet transforms \citep{donoho1995wavelets}, that have the benefit of being adaptive to the smoothness or sharpness of the signal. In settings with limited training data, these ideas can replace the automatic featurization, implicit in the representations learned by deeper architectures, with featurization partially driven by time series domain knowledge.

\subsection{Data Scarcity and Transfer Learning}

In applications with limited amounts of training data, all highly parametrized models are vulnerable to overfitting and generalize poorly.  
One known way to alleviate the problem in the univariate time series setting is by using longer periods of training data, although this may not always be feasible. 
An interesting alternative idea to explore with NBEATSx model is to optimize it in stages: first on a larger reference dataset, to then fine-tune it for the, perhaps scarce, target data  set \citep{bzinovski1976transfer_learning, pan2010transfer_survey}. 
The use of a model pre-trained on a large dataset in addition to being able to mitigate overfitting, can also help to predict for time series whose length can be short even for classical statistical methods. This is possible due to the ability of machine learning models to capture common patterns shared between correlated series.

Attempts to implement transfer learning for neural networks in the time-series domain have been limited \citep{fawaz2018transfer_ts_clf, laptev2018transfer_regloss}, but literature has shown that the results can improve or deteriorate depending on the datasets involved in the experiments. 
Yet, results attainable in computer vision domain \citep{bengio2012transfer_cv, yosinski2014transfer_how} or natural language processing \citep{quoc2017transfer_unsup_nlp, devlin2018transfer_bert} appear more systematically beneficial. This apparent discrepancy requires more investigation, and we hypothesize that different sets of data in time series domain may show less obvious similarities than databases in those more common domains of application of deep transfer learning.  
Nonetheless, this avenue of investigation remains promising.

